Posterior Consistency of Semi-Supervised Regression on Graphs

Graph-based semi-supervised regression (SSR) is the problem of estimating the value of a function on a weighted graph from its values (labels) on a small subset of the vertices. This paper is concerned with the consistency of SSR in the context of classification, in the setting where the labels have small noise and the underlying graph weighting is consistent with well-clustered nodes. We present a Bayesian formulation of SSR in which the weighted graph defines a Gaussian prior, using a graph Laplacian, and the labeled data defines a likelihood. We analyze the rate of contraction of the posterior measure around the ground truth in terms of parameters that quantify the small label error and inherent clustering in the graph. We obtain bounds on the rates of contraction and illustrate their sharpness through numerical experiments. The analysis also gives insight into the choice of hyperparameters that enter the definition of the prior.

==> SSL_Posterior_Consistency_IP_Submit (1)/ex_shared.tex <==
% SIAM Shared Information Template
% This is information that is shared between the main document and any
% supplement. If no supplement is required, then this information can
% be included directly in the main document.


% Packages and macros go here
\usepackage{amssymb}
\usepackage{bm,bbm}
\usepackage{lipsum}
\usepackage{amsfonts}
\usepackage{graphicx}
\usepackage{cite}
\usepackage{epstopdf}
\usepackage{algorithmic}
\usepackage{etoolbox}
\usepackage{stackrel}
\usepackage{multirow}
\usepackage{enumerate}
\usepackage{overpic}
\usepackage[caption=false]{subfig}
\usepackage[normalem]{ulem}

\usepackage{xr-hyper}
\makeatletter
\newcommand*{\addFileDependency}[1]{
  \typeout{(#1)}
  \@addtofilelist{#1}
  \IfFileExists{#1}{}{\typeout{No file #1.}}
}
\makeatother

\newcommand*{\myexternaldocument}[1]{
    \externaldocument{#1}
    \addFileDependency{#1.tex}
    \addFileDependency{#1.aux}
}
%%% END HELPER CODE
\usepackage{breqn}
\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi

% % fix for https://tex.stackexchange.com/questions/328946
 % \patchcmd{\SetTagPlusEndMark}{$}{}{}{}
 % \patchcmd{\SetTagPlusEndMark}{$}{}{}{}

% fix for the QED in equation*    
\renewenvironment{equation*}{\[}{\]\ignorespacesafterend}

\newcommand{\mcl}{\mathcal}
\newcommand{\mbf}{\mathbf}
\newcommand{\mbb}{\mathbb}
\newcommand{\Div}{\text{div}}
\newcommand{\dist}{\text{dist}}
\newcommand{\supp}{{\rm supp\ }}
\newcommand{\eps}{\epsilon}
\newcommand{\bD}{\bar D}
%\newcommand{\tH}{\tilde{H}}
%\newcommand{\tC}{\tilde{C}}
%\newcommand{\tPhi}{\tilde{\Phi}}
\newcommand{\tH}{H'}
\newcommand{\tC}{C'}
\newcommand{\tPhi}{\Phi'}
\newcommand{\up}{\mbf u^+}
\newcommand{\um}{\mbf u^-}
\newcommand{\Cpp}{C^{\tiny{++}}}
\newcommand{\Cmm}{C^{\tiny{--}}}
\newcommand{\Cpm}{C^{\tiny{+-}}}
\newcommand{\Cmp}{C^{\tiny{-+}}}
\newcommand{\Ppp}{P^{\tiny{++}}}
\newcommand{\Pmm}{P^{\tiny{--}}}
\newcommand{\Ppm}{P^{\tiny{+-}}}
\newcommand{\Pmp}{P^{\tiny{-+}}}

\newcommand{\tchi}{\bar{\pmb \chi}}





\newcommand{\Langle}{\left\langle}
  \newcommand{\Rangle}{\right\rangle}
\newcommand{\LLangle}{\left\llangle}
  \newcommand{\RRangle}{\right\rrangle}
\newcommand{\sgn}{\text{\rm{sgn}}}
\newcommand{\iidsim}{\stackrel{iid}{\sim}}
\newcommand{\dequal}{\stackrel{d}{=}}

\newcommand{\msf}[1]{{\mathsf #1}}
\newcommand{\blt}{\bullet}

\newcommand{\bt}{\mbf t}
\newcommand{\by}{\mbf y}
\newcommand{\bs}{\mbf s}
\newcommand{\bu}{\mbf u}
\newcommand{\br}{\mbf r}
\newcommand{\bv}{\mbf v}
\newcommand{\bz}{\mbf z}
\newcommand{\be}{\mbf e}
\newcommand{\bk}{\mbf k}
\newcommand{\ba}{\mbf a}
\newcommand{\bc}{\mbf c}
\newcommand{\bx}{\mbf x}
%\newcommand{\x}{\mbf x}
\newcommand{\dd}{\mathrm{d}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\E}{\mathcal{E}}
\newcommand{\EE}{\mathbb{E}}
\newcommand{\PP}{\mathbb{P}}
\newcommand{\pom}{{\mbf u}^{\ast}}
\newcommand{\poU}{U^\ast}
\newcommand{\poC}{C^\ast}
\newcommand{\bchi}{\bar{\bm{\chi}}}
\newcommand{\Law}{\text{Law}}
\newcommand{\bphi}{\bm{\phi}}

\newcommand{\Fnorm}[1]{\left\| #1 \right\|_F}
 
% Add a serial/Oxford comma by default.
\newcommand{\creflastconjunction}{, and~}

\newcommand{\tG}{\widetilde{G}}
\newcommand{\tW}{\widetilde{W}}
\newcommand{\tZ}{\widetilde{Z}}
\newcommand{\tN}{\widetilde{N}}
\newcommand{\tL}{\widetilde{L}}
\newcommand{\tD}{\widetilde{D}}
\newcommand{\tk}{\mathfrak{k}}
\newcommand{\biasdc}{|\poC_0 B\bu^\dagger_m/\gamma^2 - \bu^\dagger_m |}
\newcommand{\biasc}{|\poC_\epsilon B\bu^\dagger_m/\gamma^2 - \bu^\dagger_m |}

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

% Used for creating new theorem and remark environments
%\newsiamremark{remark}{Remark}
%\newsiamremark{hypothesis}{Hypothesis}
\crefname{hypothesis}{Hypothesis}{Hypotheses}
%\newsiamthm{claim}{Claim}um
\newsiamthm{assumption}{Assumption}
\newsiamthm{thm}{Theorem}

\newsiamthm{claim}{Claim}
\newsiamthm{informaldefinition}{Informal Definition}
\newsiamremark{conjecture}{Conjecture}
\newsiamremark{remark}{Remark}
\newsiamremark{example}{Example}
\newsiamremark{hypothesis}{Hypothesis}
\newsiamremark{problem}{Problem}
\crefname{hypothesis}{Hypothesis}{Hypotheses}
\AtEndEnvironment{problem}{\null\hfill$\Diamond$}
\AtEndEnvironment{example}{\null\hfill$\Diamond$}
\AtEndEnvironment{remark}{\null\hfill$\Diamond$}



% Sets running headers as well as PDF title and authors

\headers{Posterior Consistency of SSR}{A. L. Bertozzi, B. Hosseini, H. Li, K. Miller, and A. M. Stuart}



% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
% \title{Bayesian Posterior Consistency of Graph Based Semisupervised Learning\thanks{Submitted to the editors DATE.
\title{Posterior Consistency of Semi-Supervised Regression on Graphs
\thanks{Submitted to the editors DATE.
\funding{\color{black}This work is supported by NSF grant DMS 1818977, AFOSR grant FA9550-17-1-0185, NSERC PDF fellowship, a Caltech Von K{\'a}rm{\'a}n instructorship, DOD NDSEG Fellowship, and DARPA grant FA8750-18-2-0066.}}}


% Authors: full names plus addresses.
\author{
	Andrea L. Bertozzi\footnotemark[3]\and
	Bamdad  Hosseini\thanks{Computing and Mathematical Sciences, Caltech, Pasadena, CA
		(\email{bamdadh@caltech.edu}, \email{astuart@caltech.edu}).}
	\and
	Hao Li\thanks{Department of Mathematics, University of California, Los Angeles, Los Angeles, CA
		(\email{bertozzi@math.ucla.edu}, \email{lihao0809@math.ucla.edu}, \email{millerk22@math.ucla.edu}).}
	\and
	Kevin Miller\footnotemark[3]
	\and
	Andrew M. Stuart\footnotemark[2]
}


\usepackage{amsopn}
\DeclareMathOperator{\diag}{diag}


%%% Local Variables: 
%%% mode:latex
%%% TeX-master: "ex_article"
%%% End: 

